Supersymmetry production cross sections in pp collisions at sqrt{s} = 7 TeV

This document emerged from work that started in January 2012 as a joint effort by the ATLAS, CMS and LPCC supersymmetry (SUSY) working groups to compile state-of-the-art cross section predictions for SUSY particle production at the LHC. We present cross sections for various SUSY processes in pp collisions at $\sqrt{s} =7$ TeV, including an estimate of the theoretical uncertainty due to scale variation and the parton distribution functions. Further results for higher LHC centre-of-mass energies will be collected at https://twiki.cern.ch/twiki/bin/view/LHCPhysics/SUSYCrossSections. For squark and gluino production, which dominate the inclusive SUSY cross section, we employ calculations which include the resummation of soft gluon emission at next-to-leading logarithmic accuracy, matched to next-to-leading order (NLO) SUSY-QCD. In all other cases we rely on NLO SUSY-QCD predictions.

==> _region_.tex <==
\message{ !name(highOrder.tex)}
\message{ !name(highOrder.tex) !offset(-2) }
\section{Higher Order calculations -- NLO+NLL}

The inclusion of higher-order SUSY-QCD corrections is important to
reduce the dependence of the cross-section prediction on the 
renormalization and factorization scales. In general, the corrections 
also increase the size of the cross section with respect to the leading-order
prediction \cite{Kane:1982hw, Harrison:1982yi,Dawson:1983fw} if the
renormalization and factorization scales are chosen close to the
average mass of the produced SUSY particles. As a result, the
SUSY-QCD corrections have a substantial impact on the determination of
mass exclusion limits and would lead to a significant reduction of
errors on SUSY mass or parameter values in the case of discovery.  The
processes listed in Eqs.~(\ref{eq:prod}) and ~(\ref{eq:stsb_prod}) have been known for quite
some time at next-to-leading order (NLO) in
SUSY-QCD~\cite{Beenakker:1994an,Beenakker:1995fp, Beenakker:1996ch, Beenakker:1997ut}.

Following the expected squark flavor structure in the MSSM most
numerical implementations, including {\sc Prospino2}, make assumptions
about the squark mass spectrum. The left-handed and right-handed
squarks of the five light flavors are assumed to be mass
degenerate. Only the two stop masses are kept separate in the NLO
computations of light-flavor production
rates~\cite{Beenakker:1994an,Beenakker:1995fp, Beenakker:1996ch}. In
the {\sc Prospino2} implementation, this degeneracy is not assumed for
the leading-order results. However, the approximate NLO rates are
computed from the exact leading order cross sections times the mass
degenerate $K$ factor. For the pair production of third-generation
squarks the four light squark flavors are mass degenerate, while the
four third generation masses are kept
separate~\cite{Beenakker:1997ut}. This approximation can for example
be tested using {\sc MadGolem}~\cite{Binoth:2011xi}, an automized NLO
tool linked to {\sc MadGraph4}~\cite{Alwall:2007st}. It is also fitting to point out here that in {\sc Prospino2}~\cite{prospino2} the pair production of
third-generation squarks is available as individual
processes. However, sbottom pairs are included in the implicit sum of
light-flavor squarks because there is no perfect separation of bottom
and light-flavor decay jets.

When we add squark and gluino production rates including
next-to-leading order corrections it is crucial to avoid double
counting of processes. For example, squark pair production includes
$\mathcal{O}(\alpha_s^3)$ processes of the kind $qg \to \sq \sq^*
q$. The same final state can be produced in $\sq \gl$ production when
the on-shell gluino decays into an anti-squark and a quark. The {\sc
  Prospino} scheme for the separation and subtraction of on-shell
divergences from the $\sq \sq^*$ process uniquely ensures a consistent
and point-by-point separation over the entire phase space. For a
finite particle mass it has recently been adopted by {\sc MC\@@NLO}
for top quark processes. It is automized as part of {\sc
  MadGolem}~\cite{Binoth:2011xi}.



A significant part of the NLO QCD corrections can be attributed to the
threshold region, where the partonic centre-of-mass energy is close to
the kinematic production threshold. In this case the NLO
corrections are typically large, with the most significant
contributions coming from soft-gluon emission off the coloured
particles in the initial 
and final state. The contributions due to soft gluon emission can be
consistently taken into 
account to all orders by means of threshold resummation. In this
paper, we discuss results where resummation has been performed at 
next-to-leading logarithmic (NLL) accuracy~\cite{Kulesza:2008jb,Kulesza:2009kq,
Beenakker:2009ha,Beenakker:2010nq,Beenakker:2011fu}. 

The step from NLO to NLO+NLL is achieved by calculating the NLL-resummed partonic cross section $\tilde \sigma^{\rm (NLL)}$ and then matching it to the NLO prediction, in order to retain the available information on other than soft-gluon contributions. The matching procedure takes the following form
\begin{eqnarray}
\label{eq:matching}
\si^{\rm (NLO+NLL)}_{p p \to kl}\bigl(\rho, \{m^2\},\mu^2\bigr) 
  &=& \si^{\rm (NLO)}_{p p \to kl}\bigl(\rho, \{m^2\},\mu^2\bigr)\nn
          \\[1mm]
   &&  \hspace*{-30mm}+\, \frac{1}{2 \pi i} \sum_{i,j=q,\bar{q},g}\, \int_\mathrm{CT}\,dN\,\rho^{-N}\,
       \tilde f_{i/p}(N+1,\mu^2)\,\tilde f_{j/p}(N+1,\mu^2) \nn\\[0mm]
   && \hspace*{-20mm} \times\,
       \left[\tilde\si^{\rm(NLL)}_{ij\to kl}\bigl(N,\{m^2\},\mu^2\bigr)
             \,-\, \tilde\si^{\rm(NLL)}_{ij\to kl}\bigl(N,\{m^2\},\mu^2\bigr)
       {\left.\right|}_{\scriptscriptstyle({\NLO})}\, \right]\,,
\end{eqnarray}
where the last term in the square brackets denotes the NLL resummed
expression expanded to NLO. The symbol $\{m^2\}$ stands for all masses entering the calculations and  $\mu$ is the common factorization and
renormalization scale. The resummation is performed in the Mellin moment $N$ space, with all Mellin-tarnsformed quantities indicated by tilde. In particular, the Mellin moments of the partonic cross sections are defined as 
\begin{equation}
\label{eq:Mellin}
  \tilde\si_{i j \to kl}\bigl(N, \{m^2\}, \mu^2 \bigr) 
 \equiv \int_0^1 d\rhohat\;\rhohat^{N-1}\;
           \si_{ i j\to kl}\bigl(\rhohat,\{ m^2\}, \mu^2 \bigr) \,.
\end{equation}
The variable $\rhohat \equiv (m_k + m_l)^2/\shat $ measures the closeness to the partonic production threshold and is related to the corresponding hadronic variable $\rho = \rhohat x_i x_j$ in~(\ref{eq:matching}), where $x_i\ (x_j)$ are the usual longitudinal momentum fraction of the incoming proton carried out by the parton $i (j)$. The necessary inverse Mellin transform in~(\ref{eq:matching}) is performed  along the contour ${\rm CT}$ according to the so-called ``minimal prescription''~\cite{Catani:1996yz}.
The NLL resummed cross section in
Eq.~(\ref{eq:matching}) reads
\begin{eqnarray}
  \label{eq:NLLres}
  \tilde{\sigma}^{\rm (NLL)} _{ij\rightarrow kl}\bigl(N,\{m^2\},\mu^2\bigr) 
& = &\sum_{I}\,
      \tilde\sigma^{(0)}_{ij\rightarrow kl,I}\bigl(N,\{m^2\},\mu^2\bigr)\,  \\[1mm]
   & \times\,& \Delta^{\rm (NLL)}_i (N+1,Q^2,\mu^2)\,\Delta^{\rm (NLL)}_j (N+1,Q^2,\mu^2)\,
     \Delta^{\rm (s, \NLL)}_{ij\rightarrow
       kl,I}\bigl(N+1,Q^2,\mu^2\bigr)\,,
\end{eqnarray}
where the hard scale $Q^2$ is taken as $Q^2 = (m_k + m_l)^2$ and $\tilde{\sigma}^{(0)}_{ij \rightarrow kl, I}$ are the
colour-decomposed leading-order cross sections in Mellin-moment space,
with $I$ labelling the possible colour
structures~\cite{}.  The functions $\Delta^{\rm (NLL)}_{i}$ and $\Delta^{\rm (NLL)}_{j}$ sum
the effects of the (soft-)collinear radiation from the incoming
partons. They are process-independent and do not depend on the colour
structures.  These functions contain both the leading logarithmic as well
as part of the subleading logarithmic behaviour. The expressions for
$\Delta^{\rm (NLL)}_{i}$ and $\Delta^{\rm (NLL)}_{j}$ can be found in the
literature~\cite{}. In order to perform resummation at NLL accuracy, one also has to take into account soft-gluon contributions involving emissions from the final state, depending on the colour structures in which the
final state SUSY particle pairs can be produced. They are summarized by the factor
\begin{equation}
  \Delta_{I}^{\rm (s, \NLL)}\bigl(N,Q^2,\mu^2\bigr) 
  \;=\; \exp\left[\int_{\mu}^{Q/N}\frac{dq}{q}\,\frac{\alpha_{\rm s}(q)}{\pi}
                 \,D_{I} \,\right]\,.
\label{eq:2}
\end{equation}
The one-loop coefficients $D_{I}$ follow from the threshold limit of
the one-loop soft anomalous-dimension
matrix and can be found in~\cite{Kulesza:2009kq,Beenakker:2009ha}. 

The analytic results for the NLL part of the cross sections have been implemented into a numerical code. The results of this code, added to the NLO results obtained from {\sc PROSPINO}, correspond to the matched NLO+NLL cross sections, Eq.~\ref{eq:matching}. Their central values, as well as the scale, pdf and $\alpha_s$ uncertainties obtained with CTEQ6.6 and MSTW2008 pdfs have been tabulated for the squark and gluino production processes of interest in the range of input masses appropriate for the current experimental analysis. The set of tabulatd values has enough granularity in order to minimize the interpolation uncertainty when an intermediate value is used as input in the analysis. Together with a corresponding interpolation code, the tabulated values constitute the {\tt NLL-fast} numerical package~\cite{Beenakker:2011fu,nllfast}.

Note that for specific processes, results beyond NLL accuracy are
already available. The production of squark-antisquark pairs has been 
calculated at next-to-next-to-leading-logarithmic (NNLL) level 
\cite{Beenakker:2011sf}. Also, a general
formalism has been developed in the framework of effective field
theories which allows for the resummation of soft and Coulomb gluons
in the production of coloured
sparticles~\cite{Beneke:2009rj,Beneke:2010da} and subsequently applied to squark and gluino production~\cite{Beneke:2010da, Falgari:2012hx}. 
In addition, the dominant next-to-next-to-leading order (NNLO) corrections, including
those coming from the resummed cross section at
next-to-next-to-leading-logarithmic (NNLL) level, have been calculated
for squark-antisquark pair-production
\cite{Langenfeld:2009eg,Langenfeld:2010vu}. 
The production of gluino
bound states as well as bound-state effects in gluino-pair and
squark-gluino production
has also been studied \cite{Hagiwara:2009hq,Kauth:2009ud,Kauth:2011vg,Kauth:2011bz}. 
Furthermore, electroweak corrections to the ${\cal O} (\alpha_{\rm s}^2)$ tree-level
processes~\cite{Hollik:2008yi, Hollik:2008vm, Beccaria:2008mi,
    Mirabella:2009ap, Germer:2010vn, Germer:2011an} and the
electroweak Born production channels of ${\cal O} (\alpha\alpha_{\rm s})$
and ${\cal O} (\alpha^2)$~\cite{Alan:2007rp,Bornhauser:2007bf} are in
general significant for the pair production of SU(2)-doublet squarks
$\tilde{q}_L$ and at large invariant masses, but they are moderate for
inclusive cross sections and will not be included in the results
presented here. 


{\em Summary of other developments on the theory side: resummed predictions from SCET including Coulomb corrections, NNLL, NNLO-approx., NLO EW}

\message{ !name(highOrder.tex) !offset(-155) }

